eUDS: The SRG/eROSITA X-ray Survey of the UKIDSS Ultra Deep Survey Field. Catalogue of Sources

The eROSITA X-ray telescope on board the Spectrum-Roentgen-Gamma (SRG) spacecraft observed the field of the UKIDSS Ultra-Deep Survey (UDS) in August-September 2019, during its flight to Sun-Earth L2 point. The resulting eROSITA UDS (or eUDS) survey was thus the first eROSITA X-ray imaging survey, which demonstrated the capability of the telescope to perform uniform observations of large sky areas. With a moderate single-camera exposure of 150 ks, eUDS covered ~5 deg^2 with the limiting flux ranging between 4E-15 and 5E-14 erg/s/cm^2, in the 0.3-2.3 keV band. We present a catalogue of 647 sources detected at likelihood >10 (~4 sigma) during the eUDS. The catalogue provides information on the source fluxes in the main energy band 0.3-2.3 keV and forced photometry in a number of bands between 0.3 and 8 keV. Using the deeper 4XMM-DR12 catalogue, we have identified 22 strongly variable objects that have brightened or faded by at least a factor of ten during the eROSITA observations compared to previous observations by XMM-Newton. We also provide a catalogue of 22 sources detected by eROSITA in the hard energy band of 2.3-5 keV.

==> reply.tex <==
We would like to thank the reviewer for helpful suggestions. We have tried to address all of them. In some places, we had indeed missed important points. Below you can find our replies to the reviewer's comments. The corresponding changes in the text are marked in bold.

Reviewer's Comments:

This is an interesting piece of work showing the SRG/eROSITA X-ray Survey of the UKIDSS Ultra Deep Survey Field and comparing the detections to other X-ray catalogues, notably 4XMM-DR12, which is particularly pertinent in the framework of the transient sky, as the studies span almost 20 years. Whilst the study is well presented, it would be interesting to include at least a short study on the properties of the variable sources, which are the focus of this paper, for example providing an example of a long term lightcurve or a spectrum or the variable sources plotted on a colour-colour plot and/or some information on the variability over the eRosita long observation. A few details on the nature of the sources that do not have any identification (tables A1 and A4), through cross-correlating the positions with a catalogue of galaxies to understand if they are extra-galactic and if they are coincident with the centre of a galaxy, which could indicate AGN activity or possibly a tidal disruption event, or cross-correlating with Gaia could also help determine if the source is a star, for example. There is a wealth of multi-wavelength catalogues that could help with such a study. This is not a request for a detailed study, but I think adding some extra information could help to demonstrate the potential for science with this dataset and future eRosita catalogues. There are a few minor points that I also list below in the order that they appear in the text.

Authors: In the original version of this paper, we had already cross-correlated two subsamples of the eUDS catalogue, namely those reported in Tables A3 and A4, with external catalogs to search for counterparts. As suggested by the reviewer, we have now also carried out a similar analysis for the subsample presented in Table A1 and double-checked the classifications for the sources in Tables A3 and A4. This resulted in a number of additional and improved identifications. However, we should emphasise that our cross-correlation analysis so far has been aimed at revealing highly likely associations, namely with objects that are known to be AGN or Gaia stars. We plan to conduct a more careful cross-correlation analysis for the whole eUDS catalogue, using the plethora of available multi-wavelength deep photometric and spectroscopic data in the follow-up paper devoted to the eUDS survey.

Authors: Regarding a short study on the properties of the variable sources, originally we considered the possibility of providing light curves, based on XMM and eROSITA data. Hovewer, light curves based on sparce measurements (few XMM observations and one eROSITA measurement) would not look spectacular if plotted. For this reason, we provide these light curves in tabulated form in Tables A3 and A4. Variability information within eROSITA observations will be examined in our future paper, which will present detailed spectral and variability analysis.

*** Abstract : at least 10 times --> by at least a factor of ten

Authors: Corrected.

*** In section 2 it is worth mentioning that you only analyse data from the eRosita telescope, when you describe ART-XC.

Authors: Done.

*** Figure 1 : Contours show exposure levels --> Contours (from the exterior to the interior) show increasing exposure levels

Authors: Corrected.

*** Section 3.1 : starring --> staring ??

Authors: Corrected.

*** Figure 2 : it would be helpful to provide a scale for the map, especially as it is difficult to envisage the sqrt-scale (which I guess should read square-root ?).

Authors: Done.

*** P. 4 Line 55, right column, part of the sentence is missing.

Authors: Apologies for mistaken text input. Removed.

*** Section 4.3 : Why do you use a fixed search radius and not simply something like 2 or 3 times the positional error for the 4XMM-DR12 sources and the eUDS sources?

Authors: As we now explain in the text, we use a fixed radius of 15 arcsec as a conservative error radius, which exceeds the positional error and systematics. This is reasonable for this study, as it is not significantly affected by source confusion.

*** P. 6, Line 22 : the the --> the

Authors: Corrected.

*** p. 6, line 27, table A1 : it would be interesting to give the upper limit for the XMM-Newton non-detection.

Authors: We have provided upper limits estimated using the FLIX service, as described in the Appendix.

*** p. 6, if there are 84 sources detected with both XMM-Newton and eRosita above 4e-14 erg/cm²/s and the cross match reveals 53, why are there only 30 eUDS sources that have no XMM-Newton counterpart? Shouldn't this be 31, or even more as the surveys go to a much fainter flux limit, where you note 613 eUDS sources and 3603 XMM-Newton sources.

Authors: Actually there is no discrepancy here. The quoted number of cross-matches for a flux cut of 4E-14 erg/s/cm^2 has little relation to the number of sources in Table A1, as eUDS and 4XMM-DR12 have very different sensitivities. In fact, the XMM data for this field are nearly an order of magnitude deeper than eUDS. Therefore, it is quite unlikely for eROSITA to find sources in this field that were undetected by XMM. Nevertheless, we find 30 such cases, which are listed in Table A1. For illustration, imagine if the XMM catalog were yet 100 times deeper. In such a case, there would be no records at all in Table A1. On the other hand, if we ask how many XMM sources are not detected in eUDS, we will get thousands of such sources.

*** p. 6, line 43: actually 4XMM-DR13 is the latest XMM-Newton catalogue, not 4XMM-DR12. Further, have you checked the 4XMM-DR12s or 4XMM-DR13s which is the catalogue of sources detected in stacked data?

Authors: 4XMM-DR13 was released in June 2023 when significant part of this work has been already done. We have added a comment on this in a footnote. We think that reworking all the analysis with DR13 is unnecessary since no new data have been added for the UDS field in DR13 compared to DR12. Regarding the stacked XMM data, which might help find the faintest sources, we also think that using 4XMM-DR12, which is already an order of magnitude deeper than eUDS, is sufficient for our purposes. Including a more sensitive survey would increase complexity related to source confusion.

*** Tables A3 and A4, I guess that the first line for each source, when there is more than one detection, is the average flux? If that is the case, it would be useful to specify that in the details provided at the foot of the tables.

Authors: Actually, it is the weighted mean flux over XMM observations provided by 4XMM-DR12 and converted to the 0.3-2.3 keV band. We added clarification to the table notes.

*** Table A4 : it would be interesting to give the ratio as you do for in Table A3

Authors: We have added a column with the ratio.

